Nivat's conjecture holds for sums of two periodic configurations

Nivat's conjecture is a long-standing open combinatorial problem. It concerns two-dimensional configurations, that is, maps $\mathbb Z^2 \rightarrow \mathcal A$ where $\mathcal A$ is a finite set of symbols. Such configurations are often understood as colorings of a two-dimensional square grid. Let $P_c(m,n)$ denote the number of distinct $m \times n$ block patterns occurring in a configuration $c$. Configurations satisfying $P_c(m,n) \leq mn$ for some $m,n \in \mathbb N$ are said to have low rectangular complexity. Nivat conjectured that such configurations are necessarily periodic. Recently, Kari and the author showed that low complexity configurations can be decomposed into a sum of periodic configurations. In this paper we show that if there are at most two components, Nivat's conjecture holds. As a corollary we obtain an alternative proof of a result of Cyr and Kra: If there exist $m,n \in \mathbb N$ such that $P_c(m,n) \leq mn/2$, then $c$ is periodic. The technique used in this paper combines the algebraic approach of Kari and the author with balanced sets of Cyr and Kra.

==> img/tikzpictures.tex <==
\def\tikzChristmasI
{\begin{tikzpicture}[xscale=0.22,yscale=0.22]

    % grid	
	\draw [help lines] (0,0) grid (25,20);

	% black squares
    \foreach \pt in {(1,19),(3,19),(4,19),(6,19),(7,19),(8,19),(9,19),(11,19),(12,19),(14,19),(15,19),(16,19),(17,19),(19,19),(20,19),(21,19),(22,19),(24,19),(8,18),(16,18),(21,18),(1,17),(3,17),(6,17),(8,17),(9,17),(11,17),(14,17),(16,17),(17,17),(19,17),(21,17),(22,17),(24,17),(1,16),(2,16),(3,16),(4,16),(6,16),(7,16),(8,16),(9,16),(10,16),(11,16),(12,16),(14,16),(15,16),(16,16),(17,16),(18,16),(19,16),(20,16),(21,16),(22,16),(23,16),(24,16),(3,15),(8,15),(11,15),(16,15),(19,15),(21,15),(24,15),(1,14),(3,14),(4,14),(6,14),(8,14),(9,14),(11,14),(12,14),(14,14),(16,14),(17,14),(19,14),(20,14),(21,14),(22,14),(24,14),(21,13),(1,12),(3,12),(6,12),(8,12),(11,12),(14,12),(16,12),(19,12),(21,12),(22,12),(24,12),(1,11),(2,11),(3,11),(4,11),(6,11),(7,11),(8,11),(9,11),(11,11),(12,11),(14,11),(15,11),(16,11),(17,11),(19,11),(20,11),(21,11),(22,11),(23,11),(24,11),(3,10),(8,10),(16,10),(21,10),(24,10),(1,9),(3,9),(4,9),(6,9),(8,9),(9,9),(11,9),(14,9),(16,9),(17,9),(19,9),(21,9),(22,9),(24,9),(1,8),(2,8),(3,8),(4,8),(5,8),(6,8),(7,8),(8,8),(9,8),(10,8),(11,8),(12,8),(14,8),(15,8),(16,8),(17,8),(18,8),(19,8),(20,8),(21,8),(22,8),(23,8),(24,8),(3,7),(6,7),(8,7),(11,7),(16,7),(19,7),(21,7),(24,7),(1,6),(3,6),(4,6),(6,6),(7,6),(8,6),(9,6),(11,6),(12,6),(14,6),(16,6),(17,6),(19,6),(20,6),(21,6),(22,6),(24,6),(8,5),(21,5),(1,4),(3,4),(6,4),(8,4),(9,4),(11,4),(14,4),(16,4),(19,4),(21,4),(22,4),(24,4),(1,3),(2,3),(3,3),(4,3),(6,3),(7,3),(8,3),(9,3),(10,3),(11,3),(12,3),(14,3),(15,3),(16,3),(17,3),(19,3),(20,3),(21,3),(22,3),(23,3),(24,3),(3,2),(8,2),(11,2),(16,2),(21,2),(24,2),(1,1),(3,1),(4,1),(6,1),(8,1),(9,1),(11,1),(12,1),(14,1),(16,1),(17,1),(19,1),(21,1),(22,1),(24,1)} {
    	\path [fill=darkgray] \pt rectangle +(1,1);
    }	
		
\end{tikzpicture}}


\def\tikzChristmasII
{\begin{tikzpicture}[xscale=0.24,yscale=0.24]

    \def\R{0.5774}

	% hexagons
    \foreach \pt in {(0.5,16.454),(2.5,16.454),(3.5,16.454),(4.5,16.454),(5.5,16.454),(7.5,16.454),(8.5,16.454),(10.5,16.454),(12.5,16.454),(13.5,16.454),(15.5,16.454),(16.5,16.454),(17.5,16.454),(18.5,16.454),(20.5,16.454),(21.5,16.454),(23.5,16.454),(24.5,16.454),(4.0,15.588),(17.0,15.588),(1.5,14.722),(3.5,14.722),(4.5,14.722),(6.5,14.722),(9.5,14.722),(11.5,14.722),(14.5,14.722),(16.5,14.722),(17.5,14.722),(19.5,14.722),(22.5,14.722),(24.5,14.722),(1.0,13.856),(2.0,13.856),(3.0,13.856),(4.0,13.856),(5.0,13.856),(6.0,13.856),(7.0,13.856),(9.0,13.856),(10.0,13.856),(11.0,13.856),(12.0,13.856),(14.0,13.856),(15.0,13.856),(16.0,13.856),(17.0,13.856),(18.0,13.856),(19.0,13.856),(20.0,13.856),(22.0,13.856),(23.0,13.856),(24.0,13.856),(2.5,12.990),(5.5,12.990),(10.5,12.990),(15.5,12.990),(18.5,12.990),(23.5,12.990),(0.0,12.124),(2.0,12.124),(3.0,12.124),(5.0,12.124),(6.0,12.124),(8.0,12.124),(10.0,12.124),(11.0,12.124),(13.0,12.124),(15.0,12.124),(16.0,12.124),(18.0,12.124),(19.0,12.124),(21.0,12.124),(23.0,12.124),(24.0,12.124),(1.0,10.392),(4.0,10.392),(7.0,10.392),(9.0,10.392),(12.0,10.392),(14.0,10.392),(17.0,10.392),(20.0,10.392),(22.0,10.392),(0.5,9.526),(1.5,9.526),(3.5,9.526),(4.5,9.526),(6.5,9.526),(7.5,9.526),(8.5,9.526),(9.5,9.526),(11.5,9.526),(12.5,9.526),(13.5,9.526),(14.5,9.526),(16.5,9.526),(17.5,9.526),(19.5,9.526),(20.5,9.526),(21.5,9.526),(22.5,9.526),(24.5,9.526),(0.0,8.660),(8.0,8.660),(13.0,8.660),(21.0,8.660),(0.5,7.794),(2.5,7.794),(5.5,7.794),(7.5,7.794),(8.5,7.794),(10.5,7.794),(12.5,7.794),(13.5,7.794),(15.5,7.794),(18.5,7.794),(20.5,7.794),(21.5,7.794),(23.5,7.794),(0.0,6.928),(1.0,6.928),(2.0,6.928),(3.0,6.928),(5.0,6.928),(6.0,6.928),(7.0,6.928),(8.0,6.928),(9.0,6.928),(10.0,6.928),(11.0,6.928),(12.0,6.928),(13.0,6.928),(14.0,6.928),(15.0,6.928),(16.0,6.928),(18.0,6.928),(19.0,6.928),(20.0,6.928),(21.0,6.928),(22.0,6.928),(23.0,6.928),(24.0,6.928),(1.5,6.062),(6.5,6.062),(9.5,6.062),(11.5,6.062),(14.5,6.062),(19.5,6.062),(22.5,6.062),(24.5,6.062),(1.0,5.196),(2.0,5.196),(4.0,5.196),(6.0,5.196),(7.0,5.196),(9.0,5.196),(10.0,5.196),(11.0,5.196),(12.0,5.196),(14.0,5.196),(15.0,5.196),(17.0,5.196),(19.0,5.196),(20.0,5.196),(22.0,5.196),(23.0,5.196),(24.0,5.196),(10.5,4.330),(23.5,4.330),(0.0,3.464),(3.0,3.464),(5.0,3.464),(8.0,3.464),(10.0,3.464),(11.0,3.464),(13.0,3.464),(16.0,3.464),(18.0,3.464),(21.0,3.464),(23.0,3.464),(24.0,3.464),(0.5,2.598),(2.5,2.598),(3.5,2.598),(4.5,2.598),(5.5,2.598),(7.5,2.598),(8.5,2.598),(9.5,2.598),(10.5,2.598),(11.5,2.598),(12.5,2.598),(13.5,2.598),(15.5,2.598),(16.5,2.598),(17.5,2.598),(18.5,2.598),(20.5,2.598),(21.5,2.598),(22.5,2.598),(23.5,2.598),(24.5,2.598),(4.0,1.732),(9.0,1.732),(12.0,1.732),(17.0,1.732),(22.0,1.732),(1.5,0.866),(3.5,0.866),(4.5,0.866),(6.5,0.866),(8.5,0.866),(9.5,0.866),(11.5,0.866),(12.5,0.866),(14.5,0.866),(16.5,0.866),(17.5,0.866),(19.5,0.866),(21.5,0.866),(22.5,0.866),(24.5,0.866)} {
    	\draw [fill=darkgray,color=darkgray] \pt+(30:\R) -- +(90:\R) -- +(150:\R) -- +(210:\R) -- +(270:\R) -- +(330:\R) -- cycle;
    }
		
\end{tikzpicture}}
